Lift-Attend-Splat: Bird's-eye-view camera-lidar fusion using transformers

Combining complementary sensor modalities is crucial to providing robust perception for safety-critical robotics applications such as autonomous driving (AD). Recent state-of-the-art camera-lidar fusion methods for AD rely on monocular depth estimation which is a notoriously difficult task compared to using depth information from the lidar directly. Here, we find that this approach does not leverage depth as expected and show that naively improving depth estimation does not lead to improvements in object detection performance. Strikingly, we also find that removing depth estimation altogether does not degrade object detection performance substantially, suggesting that relying on monocular depth could be an unnecessary architectural bottleneck during camera-lidar fusion. In this work, we introduce a novel fusion method that bypasses monocular depth estimation altogether and instead selects and fuses camera and lidar features in a bird's-eye-view grid using a simple attention mechanism. We show that our model can modulate its use of camera features based on the availability of lidar features and that it yields better 3D object detection on the nuScenes dataset than baselines relying on monocular depth estimation.

==> figures/buckets.tex <==
\begin{figure}
\centering
\includegraphics[width=0.45\linewidth]{images/explainability/bucketed_car_NOT_e2e.png}
\caption{The performance of lidar-only, BEVFusion \cite{liang2022bevfusion} and our method on the nuScenes validation split for the car class. Each method is divided into four buckets according to the number of lidar points in the object boxes.
\rcomment{Update figure and maybe merge.}
\jcomment{Legend needs updating, also figure needs updating to e2e}
}
\label{fig:buckets}
\end{figure}

==> figures/depth_qualitative_comparison.tex <==

\begin{figure*}
\begin{center}
    \begin{subfigure}{0.3\textwidth}
        \centering
        \includegraphics[width=.8\linewidth]{depth_images/orig.png}
        % \caption{image1}
        % \label{fig:1}
    \end{subfigure}%
    \begin{subfigure}{0.3\textwidth}
        \centering
        \includegraphics[width=.8\linewidth]{depth_images/orig.png}
        % \caption{image2}
        % \label{fig:2}
    \end{subfigure}
    \begin{subfigure}{0.3\textwidth}\quad
        \centering
        \includegraphics[width=.8\linewidth]{depth_images/orig.png}
        % \caption{image3}
        % \label{fig:3}
    \end{subfigure}
    \begin{subfigure}{0.3\textwidth}
        \centering
        \includegraphics[width=.8\linewidth]{depth_images/depthloss_100_mean.png}
        % \caption{image1}
        % \label{fig:1}
    \end{subfigure}%
    \begin{subfigure}{0.3\textwidth}
        \centering
        \includegraphics[width=.8\linewidth]{depth_images/depthloss_100_mean.png}
        % \caption{image2}
        % \label{fig:2}
    \end{subfigure}
    \begin{subfigure}{0.3\textwidth}\quad
        \centering
        \includegraphics[width=.8\linewidth]{depth_images/depthloss_100_mean.png}
        % \caption{image3}
        % \label{fig:3}
    \end{subfigure}
    \begin{subfigure}{0.3\textwidth}
        \centering
        \includegraphics[width=.8\linewidth]{depth_images/depthloss_0p1_mean.png}
        % \caption{image1}
        % \label{fig:1}
    \end{subfigure}%
    \begin{subfigure}{0.3\textwidth}
        \centering
        \includegraphics[width=.8\linewidth]{depth_images/depthloss_0p1_mean.png}
        % \caption{image2}
        % \label{fig:2}
    \end{subfigure}
    \begin{subfigure}{0.3\textwidth}\quad
        \centering
        \includegraphics[width=.8\linewidth]{depth_images/depthloss_0p1_mean.png}
        % \caption{image3}
        % \label{fig:3}
    \end{subfigure}
        \begin{subfigure}{0.3\textwidth}
        \centering
        \includegraphics[width=.8\linewidth]{depth_images/depthloss_0_mean.png}
        % \caption{image1}
        % \label{fig:1}
    \end{subfigure}%
    \begin{subfigure}{0.3\textwidth}
        \centering
        \includegraphics[width=.8\linewidth]{depth_images/depthloss_0_mean.png}
        % \caption{image2}
        % \label{fig:2}
    \end{subfigure}
    \begin{subfigure}{0.3\textwidth}\quad
        \centering
        \includegraphics[width=.8\linewidth]{depth_images/depthloss_0_mean.png}
        % \caption{image3}
        % \label{fig:3}
    \end{subfigure}
\end{center}
   \caption{Accurate monocular depth does not improve fusion performance.}
\label{fig:superviseddepthloss}
\end{figure*}

==> figures/geometrydef.tex <==
\begin{asy}[width=\textwidth]
settings.render=6;
settings.prc=false;
import three;
import graph3;
import grid3;
currentprojection=perspective(6, 3, 2);

//Draw Axes
pen thickblack = black+0.75;

//Set parameters of start corner of polar volume element
real r = 1;
real f=pi/4; //phi

real df=pi/16; //dphi
real dr=0.1;

pen thinblack = black+0.25;
pen thingrey = grey+0.25;

real gridZ = -0.5;

real minGridX = -0.2;
real maxGridX = 0.8;
real minGridY = 0.1;
real maxGridY = 1.1;
real gridDimX = 10;
real gridDimY = 10;
// grid
for(int i=0; i<=gridDimX; ++i){
	real x = minGridX + ((i / gridDimX) * (maxGridX - minGridX));
	draw((x,minGridY,gridZ)--(x,maxGridY,gridZ), thingrey);
}
for(int i=0; i<=gridDimY; ++i){
	real y = minGridY + ((i / gridDimY)* (maxGridY - minGridY));
	draw((minGridX,y,gridZ)--(maxGridX,y,gridZ), thingrey);
}

// camera grid
real minGridX = -.3;
real maxGridX = .3;
real gridY = -0.3;
real minGridZ = -0.2;
real maxGridZ = .2;
real gridDimX = 8;
real gridDimZ = 5;

// grid
real deltaX = (maxGridX - minGridX) / gridDimX;
for(int i=0; i<=gridDimX; ++i){
	real x = minGridX + i * deltaX;
	draw((x,gridY,minGridZ)--(x,gridY,maxGridZ), thinblack);
}
real deltaZ = (maxGridZ - minGridZ) / gridDimZ;
for(int i=0; i<=gridDimZ; ++i){
	real z = minGridZ + i * deltaZ;
	draw((minGridX,gridY,z)--(maxGridX,gridY,z), thinblack);
}
path3 col = (minGridX + 1*deltaX,gridY, minGridZ)--(minGridX + 2*deltaX,gridY,minGridZ)--(minGridX + 2*deltaX,gridY,maxGridZ)--(minGridX + 1*deltaX,gridY,maxGridZ)--cycle;
draw(col, blue+0.75);

real phiMinY = 0.3;
real phiMaxY = 1.0;

//phi arcs
for (int i=0; i < 9; ++i) {
    real startPhiX = -phiMinY + (2 * phiMinY * i / 8);
    real endPhiX = -phiMaxY + (2 * phiMaxY * i / 8);
    draw((startPhiX, phiMinY, 0)--(endPhiX, phiMaxY, 0), thinblack);
}

// horizon line
draw((minGridX,gridY,0)--(maxGridX,gridY,0), dashed+thinblack);

// horizon edges
draw((gridY,gridY,0)--(phiMinY,phiMinY,0), dashed+thinblack);
draw((-gridY,gridY,0)--(-phiMinY,phiMinY,0), dashed+thinblack);

// The focal point!
dot((0,0,0),black);

for (int i=0; i < 8; ++i) {
    real y = phiMinY + (i * (phiMaxY - phiMinY) / 7);
    draw((-y, y, 0)--(y, y, 0), thinblack);
}

real closeMinX = -phiMinY + (2 * phiMinY * 6 / 8);
real closeMaxX = -phiMinY + (2 * phiMinY * 7 / 8);
real farMinX = -phiMaxY + (2 * phiMaxY * 6 / 8);
real farMaxX = -phiMaxY + (2 * phiMaxY * 7 / 8);

draw((closeMinX,phiMinY,0)--(closeMaxX,phiMinY,0)--(farMaxX,phiMaxY,0)--(farMinX,phiMaxY,0)--cycle, red+0.75);

//dashed connectors
real dashedFrac = 6.5;
real dashedDY = 0.1;
int numDashes = 7;
for(int i = 0; i < numDashes; ++i) {   
    real y = phiMinY + ((phiMaxY - phiMinY) * (i + 0.5) / numDashes);
    real x = -y + (2 * y) * (dashedFrac / gridDimX);
    draw((x, y, gridZ)--(x, y, 0), dotted, arrow=Arrow3(TeXHead2, Relative(.6)));
    draw((x, y, 0)--(x, y, gridZ), dotted, arrow=Arrow3(TeXHead2, Relative(.8)));
}
\end{asy}

==> figures/overall_architecture.tex <==
\begin{figure}
\begin{tikzpicture}[scale=0.6]
% styles
\tikzset{every node/.style={thick, transform shape}}
\tikzset{lin/.style={draw,thick, rounded corners=2, fill=pink!80}}
\tikzset{trf/.style={draw,thick, rounded corners=2, fill=cyan!20}}
\tikzset{mrg/.style={draw,thick, rounded corners=2, fill=green!20}}
\tikzset{det/.style={draw,thick, rounded corners=2, fill=yellow!20}}
\tikzset{enc/.style={draw,thick, trapezium, rotate=270, minimum width=1.4cm, fill=blue!20}}
\tikzset{-/.style={thick}}
\tikzstyle{fitbox}=[draw, inner sep=6pt, dashed]
% sorry
\node (lift) [lin, minimum width=2cm, rotate=-90, anchor=north] {Lift};
\node (attend) [trf, right =of lift.north, minimum width=2cm, rotate=-90, anchor=north] {Attend};
\node (splat) [lin, right =of attend.north, minimum width=2cm, rotate=-90, anchor=north] {Splat};
\node (merge) [mrg, right =0.7cm of splat.north, minimum height=0.8cm] {Merge};
\node (projbox) [fit=(lift) (attend) (splat), fitbox] {};
\node[anchor=south west] at (projbox.north) {\hspace{0.2cm}Project};
% encoders
\node (lid encoder) [enc, left =0.7cm of lift.south, anchor=north, text width=1.2cm, align=center] {Lidar encoder};
\node (cam encoder) [enc, above =1.2cm of lift.south west, anchor=east, text width=1.2cm, align=center] {Camera encoder};
% lidar bev
\node (lidar) [left=0.4cm of lid encoder.south] {\includegraphics[width=3cm]{images/arch_imgs/lidar.png}};
% images
\node at (lidar |- cam encoder) [xshift=0.3cm, yshift=-0.3cm] {\includegraphics[width=3cm]{images/arch_imgs/cam_back_left_optical_reduced.png}};
\node (images) at (lidar |- cam encoder) {\includegraphics[width=3cm]{images/arch_imgs/cam_back_optical_reduced.png}};
\node at (lidar |- cam encoder) [xshift=-0.3cm, yshift=0.3cm] {\includegraphics[width=3cm]{images/arch_imgs/cam_front_optical_reduced.png}};
% detection head
\node (det head) [det, above=0.5cm of merge, rotate=-90, anchor=east] {Detection head};
% output
\node (out) [right =0.5cm of det head.north] {\includegraphics[width=3.5cm]{images/arch_imgs/output.png}};
% arrows
\draw [->,thick] (lift.north) -- (attend.south);
\draw [->,thick] (attend.north) -- (splat.south);
\draw [->,thick] (splat.north) -- (merge);
\draw [->,thick] (images.east) -- (cam encoder.south);
\draw [->,thick] (lidar.east) -- (lid encoder.south);
\draw [->,thick] (cam encoder.north) -| (attend.west);
\draw [->,thick] (lid encoder) -- (lift);
\draw [->,thick] (merge) -- (det head);
\draw [->,thick] (det head) -- (out.west |- det head);
%
\node (spacer) [below=1.25cm of merge.south] {};
\coordinate (elbow) at (attend |- spacer) {}; 
\draw [-,thick] (lid encoder.east) |- (elbow);
\draw [->,thick] (elbow) -| (merge);
%
\end{tikzpicture}
\caption{
Lift-Attend-Splat camera-lidar fusion architecture. See Section~\ref{sec:method} for details.
}
\end{figure}

==> figures/velocity_errors_distribution.tex <==
\begin{figure*}
\centering
    \centering
    \includegraphics[width=\linewidth]{images/velocity_errors_distributions.png}
\caption{L2 velocity errors distributions per class with 80th, 90th, 95th, 99th and 99.9th percentiles. The errors are computed on nuScenes validation set. Best viewed in colour.}
\label{fig:tracking_velocity_errors}
\end{figure*}

==> tables/ablation_frames.tex <==
\begin{table}
\centering
\begin{tabular}{lcc}
~ & mAP & NDS   \\
\hline\hline
% Merge module:                                   & ~ \\
1 frame (no TFA)     & 71.2       & 72.8        \\
2 frames             & 72.1       & 73.3        \\
3 frames             & \textbf{72.1} & \textbf{73.8} \\
\caption{\label{tab:ablation_frames}
Impact of different number of frames used for training the Temporal Feature Aggregation model on the 3D object detection performance.
}
\end{tabular}
\end{table}

